Privacy-Preserving Federated Learning over Vertically and Horizontally Partitioned Data for Financial Anomaly Detection

The effective detection of evidence of financial anomalies requires collaboration among multiple entities who own a diverse set of data, such as a payment network system (PNS) and its partner banks. Trust among these financial institutions is limited by regulation and competition. Federated learning (FL) enables entities to collaboratively train a model when data is either vertically or horizontally partitioned across the entities. However, in real-world financial anomaly detection scenarios, the data is partitioned both vertically and horizontally and hence it is not possible to use existing FL approaches in a plug-and-play manner. Our novel solution, PV4FAD, combines fully homomorphic encryption (HE), secure multi-party computation (SMPC), differential privacy (DP), and randomization techniques to balance privacy and accuracy during training and to prevent inference threats at model deployment time. Our solution provides input privacy through HE and SMPC, and output privacy against inference time attacks through DP. Specifically, we show that, in the honest-but-curious threat model, banks do not learn any sensitive features about PNS transactions, and the PNS does not learn any information about the banks' dataset but only learns prediction labels. We also develop and analyze a DP mechanism to protect output privacy during inference. Our solution generates high-utility models by significantly reducing the per-bank noise level while satisfying distributed DP. To ensure high accuracy, our approach produces an ensemble model, in particular, a random forest. This enables us to take advantage of the well-known properties of ensembles to reduce variance and increase accuracy. Our solution won second prize in the first phase of the U.S. Privacy Enhancing Technologies (PETs) Prize Challenge.

==> Extra-tex/randomforest_detailed.tex <==
\subsection{Privacy-Preserving Training}
\label{sec:priv-RDT-training}

%%%%%%%%%%%% 
% Prior Material
%%%%%%%%%%%%
% We develop a cryptographic protocol that enables SWIFT and banks to collaboratively train a random forest without learning anything about each others' private datasets. 
% A random forest is an ensemble of decision trees. A decision tree is an acyclic directed graph built using recursive partitioning of training data. The training data samples are recursively divided into subsets using \textit{tests} in each node of the tree. 
% Features (or attributes) used to build tests in decision tree nodes are conventionally chosen by employing some judiciously defined criterion, e.g., information gain. Instead of using only \textit{conventional} decision trees as \textit{base} classifiers, we propose to use a mix of conventional and \textit{random decision trees}~\cite{Fan2003_is,Geurts2006_extremely}. 
% In a random decision tree, features for the tree nodes are chosen at random instead of using a selection criterion. The structure of the decision tree (that determines which features are associated with internal nodes of the decision tree) is built independent of the training data. Training data is used only to determine labels associated with the leaf nodes of the random tree.

% We argue that random decision trees (RDTs) coupled with our cryptographic protocol provide a way to preserve privacy without sacrificing accuracy. First, we note that random forests built with RDTs have been shown to be competitive against conventional random forests even in non-private scenarios~\cite{Fan2003_is,Geurts2006_extremely,Fletcher2019_decision}. Second, RDTs are an excellent fit with privacy enhancing technologies. To highlight this, we note that, for a conventional decision tree, even the structure of the tree leaks information. For instance, suppose that a trusted third-party trains a (conventional) greedy decision tree and places beneficiary account flag feature as the root. Then, this tree structure leaks to SWIFT that beneficiary account flags are highly correlated with the transaction labels. There are two ways to reduce such a leakage in conventional greedy decision trees: (i) Use differential privacy (DP) techniques when choosing features. However, it has been shown that this negatively impacts the accuracy~\cite{Jagannathan2012_apractical}, and RDTs with DP can achieve better prediction accuracy over their greedy counterparts~\cite{Friedman2010_data,Rana2015_differentially,Fletcher2017_differentially,Fletcher2019_decision}. (ii) Use secure MPC techniques to compute information gain. However, this greatly increases the computation complexity and limits scalability, given that greedy decision trees are themselves computationally expensive~\cite{Fletcher2019_decision}. 

% \subsection{Private Random Forest}
% \label{sec:priv-RDT-protocol}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{imgs/PrivRDT_protocol_1.png}
%     \caption{High-level overview of the private decision tree protocol.}
%     \label{fig:Priv-RDT-protocol}
% \end{figure}

\noindent\underline{\textbf{End-to-End Protocol for Training (Algorithm~\ref{alg:priv-RDT-train}):}} Our end-to-end protocol for privately training a random forest is described in Algorithm~\ref{alg:priv-RDT-train}.  First, SWIFT designs the features that may include original transaction features (e.g., settlement currency) and augmented features (e.g., sender-receiver frequency). We assume that the bank features are determined a prior and are known to banks and SWIFT. SWIFT then performs pre-processing of its transactions to obtain $\TX$. 
SWIFT also selects hyperparameters for the random forest: the number of trees and the height of each tree. SWIFT then builds the structure of each RDT recursively, where a feature is selected randomly for each node and a test is selected for each tree arc. Let $\tree$ denote the acyclic directed graph corresponding to an RDT. Each internal node of $T$ corresponds to a feature $\fj{j}\in\FS\cup\FB$. Each arc (i.e., directed edge) of $\tree$ corresponds to a \textit{test} (i.e., \textit{rule}) involving the feature associated with the node attached to its tail. 
Algorithm~\ref{alg:RDT-build-label} in Appendix formally presents the steps for building a tree structure. 
% Fig.~\ref{} gives an example of the structure of an RDT. 
It is important to note that SWIFT builds tree structures independent of transaction dataset. Therefore, any tree structure does not leak any information about SWIFT dataset. A tree structure, however, leaks which features and tests are used by SWIFT. As we will see, tree structure is never shared with banks and thus they do not learn anything about SWIFT features.  


Next part is to compute labels for the leaf nodes of each tree. To obtain the label at a leaf node, it is required to compute statistics at leaves. These statistics are computed by \textit{filtering} training samples through the tree. Now, we establish some notation that will help us to describe the next steps.\footnote{In Appendix, we present a toy example for all the notation and algorithms.}
\hayim{Maybe a shorter way to describe is to ``squash'' all the paths to the leaves, so in each leaf we are left with a set of comparisons. Some comparisons SWIFT can make by its own. The rest with help of the bank.} \swanand{Thanks, Hayim. This is what is done -- SWIFT makes as many comparisons as it can with its features, and rest are done with the help of banks. Notation $\tests{\Path{L}}$ squashes all tests for the leaf node. I like you idea that we can associate a leaf node with the set of all tests, but this would involve change of notation. I will try, if time permits.}
In a tree structure $T$, we denote an internal node with its associated feature $\fj{j}$, and denote a leaf node as $L$. For a leaf node $L$, let $\Path{L}$ denote the path from the root node to $L$. Note that $\Path{L}$ is a sequence of features.
Let $\tests{\Path{L}}$ denote the set of tests associated with $\Path{L}$, and $\tests{\Path{L}\setminus\{f_j\}}$ denote the subset of $\tests{\Path{L}}$ by excluding the test corresponding to $\fj{j}$. 
Given a training set $\TX_t \subseteq \TX$, for a leaf node $L$ and $\ell\in\{0,1\}$, let $\NlL{\ell}{L}$ denote the number of transactions in $\TX_t$ with label $\ell$ that satisfy all the tests in $\tests{\Path{L}}$. If $\NlL{0}{L} \geq \NlL{1}{L}$, then $\Label{L} = 0$; else, $\Label{L} = 1$. 

For a tree structure $T$, SWIFT computes the label for every leaf $L$ for which its path from root contains features only from $\FS$, i.e., $\Path{L}\subseteq\FS$ and $\Path{L}\cap\FB = \varnothing$ (Line~\ref{line:leaf-lable-SWIFT}). For each leaf node $L$ in $T$ for which its path from root contains one or more bank features, SWIFT and banks collaborate to compute the label. The set of such leaf nodes at SWIFT is denoted as $\mathcal{S}$ (Line~\ref{line:set-S}.\todo{of which Alg?}) \todo{Swanand: added the Alg no. to the title in bold.} Next, we describe the algorithm to privately compute the labels for leaf nodes. 


\todo{ 1. write an assumption about the sub-tree not having more than one feature from the bank. 2.  Also, change notation in algo 1. ln 16}


\todo[inline]{my attempt to shorten Algorithm~\ref{alg:priv-RDT-train}, the original one is right after this new version.}

\begin{algorithm}[!h]
\caption{Private Random Forest (Training)}
\label{alg:priv-RDT-train}
{\begin{tabbing}
    \textbf{Participants:} SWIFT $S$, Banks $B_1, \ldots B_N$, (Aggregator)\\
	\textbf{Public Parameters:} a security parameter $\lambda$, dataset schema\\
% 	\quad An HE scheme $\E_A = (\Gen_A,\Enc_A,\Dec_A,\Add_A,\Mul_A).$\\
	\textbf{Input:} SWIFT feature set $\FS$ and transaction set $\TX$, the number $\tau$ and the height $h$ of trees, \\
	\quad and each bank partition feature set $\FB$\\
    \textbf{Output:} \= A random forest trained on the combined datasets
\end{tabbing}}
\vspace{-8pt}
% SWIFT designs transaction features \\
% SWIFT pre-processes transactions to obtain $\TX$ having features in $\FS$\\
% SWIFT chooses the number of trees $\tau$ and the height $h$ of a tree\\ 
SWIFT initializes the forest $\mathcal{F} \leftarrow \varnothing$, $\mathcal{L}_S \leftarrow \varnothing$, $\mathcal{L}_B \leftarrow \varnothing$, $\mathcal{S} \leftarrow \varnothing$\\
% \For{$t = 1, 2, \ldots, \tau$} {
SWIFT randomly generates the structure of a tree $T$ with depth $h$ based on $\FS, \FB$
and repeats the process $\tau$ times to obtain forest $\mathcal{F}$\\
    % $\mathcal{F} \leftarrow \mathcal{F}\cup T$
% }
\ForEach{tree $T \in \mathcal{F}$}{
    SWIFT selects a set of transactions $\TX_t\subseteq\TX$\\ %\tcp{used as training set to generate labels for $T$}
    % SWIFT initializes $\mathcal{L}_S \leftarrow \varnothing$, $\mathcal{L}_B \leftarrow \varnothing$, $\mathcal{S} \leftarrow \varnothing$\\
    % \If{$T$ does not contain any bank feature from $\FB$}{
    %     \ForEach{leaf node $L_i \in T$}{
    %     SWIFT generates $\Label{L_i} \leftarrow \textsc{GetLeafLabel}(T, L_i, \TX_t)$ \tcp{Algorithm~\ref{alg:RDT-build-label}}
    %     }
    % }
    % \Else{
        \ForEach{leaf node $L$ in $T$}{
            \If{$\Path{L}\cap\FB = \varnothing$}{
                SWIFT generates $\Label{L}$ and updates $\mathcal{L}_S \leftarrow \mathcal{L}_S \cup (L, \Label{L})$\\
            }
            \Else{
                % SWIFT computes $\fj{b}[L_i]$, $\Acc^0[L_i]$, $\Acc^1[L_i]$ \tcp{Sec.~\ref{sec:priv-RDT}, Eq.~\eqref{eq:candidate-acc-count}}
                SWIFT updates $\mathcal{L}_B \leftarrow \mathcal{L}_B \cup (L, ?)$, $\mathcal{S} \leftarrow \mathcal{S} \cup (\TX_t, T, L)$\label{line:set-S} 
            }
        }
    % }
  }
SWIFT and Banks collaboratively run Algorithm~\ref{alg:RDT-priv-label} (along with aggregator*) to compute the labels for leaf nodes in $\mathcal{L}_B$. The output for the banks is the encrypted label for the leaf nodes.
\end{algorithm}



% \begin{algorithm}[!h]
% \caption{Private Random Forest (Training)}
% \label{alg:priv-RDT-train}
% {\begin{tabbing}
%     \textbf{Participants:} SWIFT $S$, Banks $B_1, \ldots B_N$, (Aggregator)\\
% 	\textbf{Public Parameters:} a security parameter $\lambda$, dataset schema\\
% % 	\quad An HE scheme $\E_A = (\Gen_A,\Enc_A,\Dec_A,\Add_A,\Mul_A).$\\
% 	\textbf{Input:} SWIFT has a transaction dataset and each bank has an account dataset (Section~\ref{sec:notation})\\
%     \textbf{Output:} \= A random forest trained on the combined datasets
% \end{tabbing}}
% \vspace{-8pt}
% SWIFT designs transaction features $\FS, \FB$\\
% SWIFT pre-processes transactions to obtain $\TX$ having features in $\FS$\\
% SWIFT chooses the number of trees $\tau$ and the height $h$ of a tree\\ 
% SWIFT initializes the forest $\mathcal{F} \leftarrow \varnothing$\\
% \For{$t = 1, 2, \ldots, \tau$} {
%     SWIFT generates $T \leftarrow \textsc{BuildTreeStructure}(h, \FS, \FB)$ \tcp{Algorithm~\ref{alg:RDT-build-label}}
%     $\mathcal{F} \leftarrow \mathcal{F}\cup T$
% }
% \ForEach{tree $T \in \mathcal{F}$}{
%     SWIFT selects a set of transactions $\TX_t\subseteq\TX$\\ %\tcp{used as training set to generate labels for $T$}
%     SWIFT initializes $\mathcal{L}_S \leftarrow \varnothing$, $\mathcal{L}_B \leftarrow \varnothing$, $\mathcal{S} \leftarrow \varnothing$\\
%     % \If{$T$ does not contain any bank feature from $\FB$}{
%     %     \ForEach{leaf node $L_i \in T$}{
%     %     SWIFT generates $\Label{L_i} \leftarrow \textsc{GetLeafLabel}(T, L_i, \TX_t)$ \tcp{Algorithm~\ref{alg:RDT-build-label}}
%     %     }
%     % }
%     % \Else{
%         \ForEach{leaf node $L$ in $T$}{
%             \If{$\Path{L}\cap\FB = \varnothing$}{
%                 SWIFT generates $\Label{L} \leftarrow \textsc{GetLeafLabel}(T, L, \TX_t)$ \tcp{Algorithm~\ref{alg:RDT-build-label}}\label{line:leaf-lable-SWIFT} 
%                 SWIFT appends $\mathcal{L}_S \leftarrow \mathcal{L}_S \cup (L, \Label{L})$\\
%             }
%             \Else{
%                 % SWIFT computes $\fj{b}[L_i]$, $\Acc^0[L_i]$, $\Acc^1[L_i]$ \tcp{Sec.~\ref{sec:priv-RDT}, Eq.~\eqref{eq:candidate-acc-count}}
%                 SWIFT appends $\mathcal{L}_B \leftarrow \mathcal{L}_B \cup (L, ?)$, $\mathcal{S} \leftarrow \mathcal{S} \cup (\TX_t, T, L)$\label{line:set-S} 
%             }
%         }
%     % }
%   }
% SWIFT and Banks collaboratively run Algorithm~\ref{alg:RDT-priv-label} (along with aggregator*) to compute the labels for leaf nodes in $\mathcal{L}_B$. The output for the banks is the encrypted label for the leaf nodes.
% \end{algorithm}

\vspace{0pt}
\noindent\textbf{Privately Compute Leaf Labels:} 
SWIFT begins with computing, for each set $S = (\TX_t, \tree, L)$ from $\mathcal{S}$, three quantities $\fj{b}[L]$, $\Acc^{0}[L]$, and $ \Acc^{1}[L]$ defined in the following. 

\noindent\underline{Definition of $\fj{b}[L]$:} If $\Path{L}$ in $T$ contains a bank feature; let us denote it as $\fj{b}$.
We define the \textit{bank feature associated with} $L$, denoted as $\fj{b}[L]$, to be the value\footnote{For categorical features, we consider the value of the feature. This can be extended to continuous features by considering the test or condition.} of the bank feature $\fj{b}$ on the arc outgoing from the node $\fj{b}$ that leads to leaf $L$. For example, in Fig.~\ref{}, $\fj{b}$ is the Beneficiary Account flag, and $\fj{b}[L_1] = 0$.
% For example, $\fj{b}$ can be an Ordering Account flag or a Beneficiary Account flag.


%%%%%%%%%%%%%%%%%%%%%%
% Private Label Compute
%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[!h]
\caption{Compute Private Label}
\label{alg:RDT-priv-label}
{\begin{tabbing}
    \textbf{Participants:} SWIFT $S$, Banks $B_1, \ldots B_N$, (Aggregator)\\
	\textbf{Public Parameters:} a security parameter $\lambda$, dataset schema, \\
	\quad an HE scheme $\E_S$, a hash function $\mathsf{hash}:\{0,1\}^{\sigma} \rightarrow [0, \numBins]$\\ %(\Gen_S,\Enc_S,\Dec_S,\Add_S,\Mul_S)
	\textbf{Inputs at SWIFT:} Sets $\mathcal{L}_B,\mathcal{S}$ from Algorithm~\ref{alg:priv-RDT-train}\\
	\textbf{Inputs at Banks:} Bank $B_j$ has set $\Acc_{B_j}$ of pairs of account number and its flag\\
    \textbf{Output:} Each bank gets encrypted labels\\
    \textbf{Setup:} SWIFT generates a key-pair $(\sk, \pk)$ for HE $\E_S$ and shares $\pk$ with all banks
\end{tabbing}}

\vspace{-4pt}
\ForEach{set $S \in \mathcal{S}$}{
    SWIFT unpacks $(\TX_t, T, L_i) \leftarrow S$\\
    SWIFT computes $\fj{b}[L_i], \Acc^{0}[L_i], \Acc^{1}[L_i]$  \tcp{Defined in Section~\ref{sec:priv-RDT-protocol}}
}
SWIFT arbitrarily orders and indexes $m:=|\mathcal{L}_B|$ leaf nodes to obtain $\mathcal{L}_B = [L_1, L_2, \ldots, L_m]$\\
SWIFT computes encrypted hash tables
$\{(\en{\hashTable^{0}_{L_i}},\en{\hashTable^{1}_{L_i}}\}_{i=1}^{m} \leftarrow \textsc{GetEncHashTables}\left(\{\Acc^{0}[L_i],\Acc^{1}[L_i]\}_{i=1}^{m}\right)$\tcp{Algorithm~\ref{alg:get-enc-hash-tables}}\label{line:compute-enc-hash-tables}
\ForEach{$i =1$ to $m$}{\label{line:start-loop-compute-enc-count}
    \ForEach{$\ell\in\{0,1\}$}{
        SWIFT sends $(\textrm{leaf index } i, \ell, \en{\fj{b}[L_i]}, \en{H^{\ell}_{L_i}})$  to all banks

        \ForEach{$j = 1$ to $N$}{
            Bank $B_j$ receives $(\textrm{leaf index } i, \ell, \en{\fj{b}[L_i]}, \en{H^{\ell}_{L_i}})$\\
            $\chi_{B_j} \leftarrow 0$\\
            \ForEach{$\flag \in $ domain of flags}{
                $B_j$ computes set of accounts $\Acc_{B_j}^{\flag}$ that have flag value $\flag$\\
                % \ForEach{$\Acck{k} \in \Acc_{B_j}^{\flag}$}{
                %     $\chi_{B_j} \leftarrow \chi_{B_j} + \left(\sum_{j=1}^{\mathsf{numBins}} \PET{\en{\hashTable^{\ell}_{L_i}[\hash{\Acck{k}}, j][1]}}{\hash{\Acck{k}}} \cdot \en{\hashTable^{\ell}_{L_i}[\hash{\Acck{k}}, j][2]}\right)\cdot\PET{\en{\fj{b}[L_i]}}{\flag}$\\
                % }
                $\chi_{B_j} \leftarrow \chi_{B_j} + \sum_{\Acck{k}\in\Acc_{B_j}^{\flag}} \left(\sum_{j=1}^{\mathsf{numBins}} \PET{\en{\hashTable^{\ell}_{L_i}[\hash{\Acck{k}}, j][1]}}{\hash{\Acck{k}}} \cdot \en{\hashTable^{\ell}_{L_i}[\hash{\Acck{k}}, j][2]}\right)\cdot\PET{\en{\fj{b}[L_i]}}{\flag}$
            }
          Bank $B_j$ generates additive secret shares of $\chi_{B_j}$ as $\chi_{B_j}^{(1)}$ and $\chi_{B_j}^{(2)}$, sends $(i, \ell, \chi_{B_j}^{(1)})$ to SWIFT and $(i, \ell, \chi_{B_j}^2)$ to the other banks
        }
        SWIFT receives from banks $\{(i, \ell, \chi_{B_j}^{(1)})\}_{j=1}^{N}$, computes $\chi^{(1)} := \sum_{j=1}^{N}\chi_{B_j}^{(1)}$ and sends $(i, \ell, \chi^{(1)})$ to all banks\\
        Each bank receives from other banks $\{(i, \ell, \chi_{B_j}^{(1)})\}_{j=1}^{N}$ and $(i, \ell, \chi^{(1)})$ from SWIFT\\ 
        Each bank computes $\chi^{\ell}_{L_i} := \sum_{j=1}^{N}\chi_{B_j}^{(2)} + \chi^{(1)}$, and stores $(i, \ell, \chi^{\ell}_{L_i})$ 
        \tcp{We prove that $\chi^{\ell}_{L_i} = \en{\NlL{\ell}{L_i}}$} 
    }\label{line:end-loop-compute-enc-count}
    Each bank $B_j$ computes $\en{\Label{L_i}} \leftarrow 2\cdot\en{\chi^{0}_{L_i} \lessgtr \chi^{1}_{L_i}}-1$, and stores $(i, \en{\fj{b}[L_i]}, \en{\Label{L_i}})$
}
\textbf{Output:} SWIFT gets a list of nodes $\mathcal{L}_B = [L_1, L_2, \ldots, L_m]$ whose path includes a bank feature; Each bank gets $\left\{(i, \en{\fj{b}[L_i]}, \en{\Label{L_i}}\right\}_{i=1}^{m}$
\end{algorithm}


% \begin{algorithm}[!h]
% \caption{Get Encrypted Hash Tables}
% \label{alg:get-enc-hash-tables}
% \textbf{procedure:} \textsc{GetEncHashTables}$\left(\{\Acc^{0}[L_i],\Acc^{1}[L_i]\}_{i=1}^{m}\right)$\\
% \textbf{parameters:} hash function $\mathsf{hash}:\{0,1\}^{\sigma}\rightarrow[1,\numBins]$, an HE key-pair $(\sk,\pk)$\\
% \ForEach{$i=1$ to $m$}{
%     \ForEach{$\ell\in\{0,1\}$}{
%         Initialize hash table $\hashTable^{\ell}_{L_i}$ with $\numBins$ empty bins \tcp{$\hashTable^{\ell}_{L_i}[p]$ denotes $p$-th bin}
%         \ForEach{$(\Acck{k},c_k) \in \Acc^{\ell}[L_i])$}{
%             Append the bin $\hashTable^{\ell}_{L_i}[\hash{\Acck{k}}]$ with $({\hash{\Acck{k}}}, {c_k})$\\
%         }
%     }
% }
% Compute $\binSize \leftarrow$ maximum number of pairs in a bin across all hash tables\\
% Pad bins as necessary with $(\hash{\textrm{dummy account number}}, 0)$ so that every bin in each hash table has $\binSize$ pairs\\ 
% Encrypt every pair in each hash table using $\pk$ of $\E_S$ \tcp{After encryption, an element in a bin will be of the form $(\en{\hash{\Acck{k}}}, \en{c_k})$}
% \Return{$\{(\en{\hashTable^{0}_{L_i}},\en{\hashTable^{1}_{L_i}}\}_{i=1}^{m}$}\\
% \textbf{end procedure}
% \end{algorithm}



\noindent\underline{Definitions of $\Acc^{0}[L_i]$, $\Acc^{1}[L_i]$:} \todo{previously we don't have the subscript $i$, shall we remove it here?} Let $\TX_t^{\ell}$ denote the set of transactions from $\TX_t$ with label $\ell \in\{0,1\}$. 
% For a node $v$ of $T$ (which can be either an internal node or a leaf node), let $\TX_t^{\ell}[v]$ denote the set of transactions from $\TX_t^{\ell}$ that \textit{filter} out to $v$, i.e, the transactions that satisfy all the tests in $\tests{\Path{v}}$
We define the set of \textit{candidate transactions} $\TX_t^{\ell}[L_i] \subseteq \TX_t$ that can reach $L_i$. More formally, $\TX_t^{\ell}[L_i]$ is the set of transactions that satisfy all the tests in $\tests{\Path{L_i}\setminus\{\fj{b}\}}$ given as
\begin{equation}
    \label{eq:candidate-tx}
        \TX_t^{\ell}[L_i] = \left\{ \txi{i}\in\TX_t^{\ell} : \txi{i} \textrm{ satisfies all the tests in } \tests{\Path{L_i}\setminus\{\fj{b}\}}\right\}.
\end{equation}

For an account number $\Acck{k}$, we define $\Count_{\fj{b}}(a_k, \TX_t^{\ell}[L_i])$ to be the number of times $a_k$ appears in the transactions in $\TX_t^{\ell}[L_i]$ corresponding to feature $\fj{b}$. For instance, if $\fj{b}$ is a Beneficiary Account flag, then $\Count_{\fj{b}}(\Acck{k}, \TX_t^{\ell}[L_i])$ denotes the number of transactions in $\TX_t^{\ell}[L_i]$ in which $\Acck{k}$ appears as a Beneficiary Account.  This allows us to define a set of \textit{candidate accounts with counts} as the set pairs of account number and its count for all accounts appearing the transactions in $\TX_t^{\ell}[L_i]$ for $\ell\in\{0,1\}$ as follows:
\begin{equation}
    \label{eq:candidate-acc-count}
        \Acc^{\ell}[L_i] = \left\{ (\Acck{k}, c_k) : \Acck{k} \textrm{ appears in } \txi{i} \textrm{ under } \fj{b}, \txi{i}\in\TX_t^{\ell}[L_i] \right\}, \: c_k := \Count_{\fj{b}}(\Acck{k}, \TX_t^{\ell}[L_i]).
\end{equation}
% Next, we define a partition $\Acc^{\ell}[L_i] = \cup_{j=1}^{N} \Acc^{\ell}_{B_j}[L_i]$, where $\Acc^{\ell}_{B_j}[L_i]$ contain all pairs from  $\Acc^{\ell}[L_i]$ for which the accounts belong to bank $B_j$. That is, we have
% \begin{equation}
%     \label{eq:candidate-acc-count-bank}
%         \Acc^{\ell}_{B_j}[L_i] = \left\{ (\Acck{k}, c_k) : (\Acck{k}, c_k)\in\Acc^{\ell}[L_i] \textrm{ and } \Acck{k} \in \Acc_{B_j}.\textsf{accounts} \right\}.
% \end{equation}
% Note that $\Acc^{\ell}_{B_j}[L_i]$ may be empty for certain banks $B_j$.

Next, on Line~\ref{line:compute-enc-hash-tables} of Algorithm~\ref{alg:RDT-priv-label}, SWIFT computes encrypted hash tables using Algorithm~\ref{alg:get-enc-hash-tables}. Every hash table $\en{\hashTable^{\ell}}$ has $\numBins$ bins. Note that, due to padding (with dummy accounts and zero counts) in Algorithm~\ref{alg:get-enc-hash-tables}, each bin contains $\binSize$ elements. We denote $j$-th element in $i$-th bin as $\en{\hashTable^{\ell}}[i][j]$, where each element is of the form $(\en{\Acck{k}}, \en{c_k})$. 

On Lines~\ref{line:start-loop-compute-enc-count} to~\ref{line:end-loop-compute-enc-count}, SWIFT and Banks collaborate so that, for each leaf node $L_i$ and label $\ell$, every bank obtains a value $\chi^{\ell}_{L_i}$. Later, while proving the correctness of the protocol, we prove that $\chi^{\ell}_{L_i} = \en{\NlL{\ell}{L_i}}$. In this process, we utilize a Private Equality Test $\mathsf{PET}$. We use binary representation for hash values, encrypt each bit in a ciphertext slot, and realize $\PET{ct}{pt}$ as a binary circuit $\left(\prod_i 1 - (ct_i - pt_i)\right)^2$. \todo{Hayim/Nir/Eyal, could you please check and add details?}
\todo{It is more efficient to compute $(\Pi_i (1-ct_i - pt_i))^2$ I think Allon Adir has a patent about it. We can cite it here. I'll ask him.}
Finally, each bank computes an (approximate)\hayim{why approximate? You can use BGV or BFV} comparison under HE to obtain encrypted label for each leaf node. \todo{Hayim/Nir/Eyal, can you please add references for comparison circuit that we have in HELayers? It needs an upper bound on absolute difference between counts. This can be bounded to 1 if counts are normalized by total number of accounts. We may need to add that step.}
\todo{If you are going with CKKS, I think it is best to cite "Efficient Homomorphic Comparison Methods
with Optimal Complexity" or "BLEACH: Cleaning Errors in DiscreteComputations over CKKS" that was recently submitted}

\vspace{0pt}
\noindent\textbf{Model at the end of training:} After executing the training protocol Algorithm~\ref{alg:priv-RDT-train}, SWIFT has the random forest $\mathcal{F}$ with tree structures. The leaf nodes of the forest are partitioned into two sets $\mathcal{L}_S$ and $\mathcal{L}_B$. For leaf nodes in $\mathcal{L}_S$, whose path includes only SWIFT features $\FS$, the labels are with SWIFT. For leaf nodes in $\mathcal{L}_B$, whose path includes a bank feature (along with SWIFT features), every bank possesses its label under HE encryption. SWIFT holds the secret key for the encryption, and thus the banks learn no information about any label.

\subsection{Privacy-Preserving Inference}
\label{sec:priv-RDT-inference}
Let us consider the case when SWIFT gets an unlabeled transaction $\tx$, and wants to predict its label. Algorithm~\ref{alg:priv-RDT-inference} describes the protocol for inference. At a high-level, the algorithm computes the label for every tree in the forest and then takes the majority vote. The confidence is the fraction of the count of the majority class divided by the number of trees. 

Now, we describe how to obtain a label for a tree $T\in\mathcal{F}$. SWIFT traverses $\tx$ through $T$, starting with the root node and following the arc according to which test passes. For instance, suppose the root node is associated with the feature currency. If $\tx$ is in Euro, then continue to the child node attached to arc with value Euro. 

There are two cases possible during the traversal. In Case 1 (i.e., branch corresponding to Line~\ref{line:leaf-in-LS}, $\tx$ does not encounter any bank feature and reaches a leaf node in $\mathcal{L}_S$. Since SWIFT has labels for the nodes in $\mathcal{L}_S$, SWIFT obtains the label the tree $T$ and continues to the next tree. 

In Case 2 (i.e., branch corresponding to Line~\ref{line:leaf-in-LB}), $\tx$ reaches an internal node in $T$ associated with a bank feature $\fj{b}$. In this case, SWIFT cannot continue the tree traversal because it does not know the value of the bank feature in $\tx$. 

Let us denote the set of leaf nodes of $T'$ as $\leafNodes{T'}$. Transaction $\tx$ can reach any leaf from $\leafNodes{T'}$ for which it satisfies all the tests associated with SWIFT features. We call such a set as \textit{candidate leaf nodes}. Formally, for a subtree $T'$ of $T$ rooted on $\fj{b}$, the set of candidate leaf nodes for $\tx$ is defined as
\begin{equation}
    \label{eq:candidate-leaf-nodes}
       \C{T'}{\tx} = \left\{L_i \in \leafNodes{T'} : \tx \textrm{ satisfies all tests in } \tests{\Path{L_i}\setminus\{\fj{b}\}} \right\}.
\end{equation}
Note that $\C{T'}{\tx} \subseteq \mathcal{L}_B$. Let $L_{i_1}, L_{i_2}. \ldots, L_{i_{m'}}$ be the nodes in $\mathcal{L}_B$ corresponding to $\C{T'}{\tx}$.

SWIFT extracts the account number $\Acck{k^*}$ from $\tx$ corresponding to $\fj{b}$ (Line~\ref{line:acc-in-tx}). For example, if $\fj{b}$ is Ordering Account Flag, then SWIFT will extract the account number of Ordering Account from $\tx$. SWIFT sends the encrypted hash of $\Acck{k^*}$ along with the indices of the candidate leaf nodes ${i_1}, {i_2}. \ldots, {i_{m'}}$ to bank $B_{j^*}$ that holds $\Acck{k^*}$ (Line~\ref{line:SWIFT-to-bank-tuple}). We note here that, if SWIFT does not know which bank would possess $\Acck{k^*}$, then it can send the tuple to all banks, and all banks follow the steps in Lines~\ref{line:bank-steps-start} to~\ref{line:bank-steps-end}. However, for the ease of exposition, we do not focus on this scenario.

The key computation at the bank is Line~\ref{line:FHE-PET-inference}, wherein it compares $\en{\hash{\Acck{k^*}}}$ received from SWIFT with the hash of each of its accounts with a specific flag. Later, when proving the correctness, we prove that on Line~\ref{line:chi-from-bank}, $\chi$ computed by the bank equals the encrypted label of the \textit{correct} leaf node to which $\tx$ would reach.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Inference 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[!h]
\caption{Inference for Private Random Forest}
\label{alg:priv-RDT-inference}
{\begin{tabbing}
    \textbf{Participants:} SWIFT $S$, Banks $B_1, \ldots B_N$, (Aggregator)\\
	\textbf{Public Parameters:} a security parameter $\lambda$, dataset schema\\
% 	\quad An HE scheme $\E_A = (\Gen_A,\Enc_A,\Dec_A,\Add_A,\Mul_A).$\\
	\textbf{Inputs at SWIFT:} a transaction $\tx$ for prediction, Features $\FS, \FB$,\\ 
	\quad random forest $\mathcal{F}$, lists of leaf nodes $\mathcal{L}_S$, $\mathcal{L}_B$, labels for leaf nodes in $\mathcal{L}_S$\\
	\textbf{Inputs at Banks:} Each bank has $\{(i, \en{\fj{b}[L_i}, \en{\Label{L_i})} : L_i\in\mathcal{L}_B\}$,\\ 
	\quad Each bank $B_j$ has the set $\Acc_{B_j}$ of pairs of account number and its flag\\
    \textbf{Output:} \= Label for $\tx$ along with a confidence score
\end{tabbing}}

\vspace{-4pt}
SWIFT pre-processes $\tx$ to obtain its features as in $\FS$\\
SWIFT initializes the label set $\mathcal{Y}\leftarrow\varnothing$\\
\ForEach{tree $T \in \mathcal{F}$}{\label{line:leaf-in-LS}
    SWIFT \textit{filters} out $\tx$ through $T$\\
    \If{$\tx$ reaches a leaf node $L \in \mathcal{L}_S$}{
        \tcc{In this case, $\tx$ does not encounter any bank feature from $\FB$}
        SWIFT retrieves $\Label{T} \leftarrow \Label{L}$, and augments
        $\mathcal{Y} \leftarrow \mathcal{Y} \cup \Label{T}$\\
    }
    \Else{\label{line:leaf-in-LB}
            \tcc{In this case, $\tx$ encounters a node with bank feature $\fj{b}$, and it will reach at one of the leaf nodes in $\mathcal{L}_B$}
            SWIFT retrieves the account $\Acck{k^*}\in\tx$ corresponding to $\fj{b}$\label{line:acc-in-tx}\\
            SWIFT computes, for the subtree $T'$ of $T$ rooted on $\fj{b}$, the set $\C{T'}{\tx}$ of candidate leaf nodes for $\tx$ \tcp{Defined in Section~\ref{sec:priv-RDT-protocol}}
            SWIFT retrieves the corresponding $m' := |\C{T}{\tx}|$ leaf nodes from $\mathcal{L}_B$ as $L_{i_1}, L_{i_2}, \ldots, L_{i_{m'}}$\\
            SWIFT sends  $(\en{\hash{\Acck{k^*}}}, \{i_1, i_2, \ldots, i_{m'}\})$ to bank $B_{j^*}$ that contains $\Acck{k^*}$\label{line:SWIFT-to-bank-tuple} \tcp{If SWIFT does not know which bank to send, it sends to all banks}
            \textbf{Bank $B_{j^*}$ performs:}\label{line:bank-steps-start}\\
            \quad Bank sets $\chi \leftarrow 0$\\
            \quad \ForEach{$p = 1$ to $m'$}{
                \quad  \ForEach{$\flag \in $ domain of flags}{
                    \quad Bank computes set of accounts $\Acc_{B_{j^*}}^{\flag}$ that have flag value $\flag$\\
                    \quad $\chi \leftarrow \chi + \left(\sum_{\Acck{k}\in\Acc_{B_{j^*}}^{\flag}} \PET{\en{\hash{\Acck{k^*}}}}{\hash{\Acck{k}}}  \right)\cdot\PET{\en{\fj{b}[L_{i_p}]}}{\flag} \cdot \en{\Label{L_{i_p}}}$\label{line:FHE-PET-inference}
                    }
            }
            \quad Bank sends $\chi$ to SWIFT\label{line:bank-steps-end}\label{line:chi-from-bank} \tcp{We prove that $\chi = \en{\Label{L_{i_*}}}$, where $L_{i_*}$ is the leaf node in $T$ to which $\tx$ reaches}
            SWIFT receives $\chi$, decrypts it with $\sk$ to obtain $\Label{T}$, and appends $\mathcal{Y} \leftarrow \mathcal{Y} \cup \Label{T}$
         }
}
SWIFT outputs the majority label from $\mathcal{Y}$ as the label for $\tx$ with confidence equal to the fraction of the majority
\end{algorithm}


\subsection{Differential Privacy for Protecting against Inference-Time Attacks}
\label{sec:DP}





==> attacks-not-used.tex <==
\section{Security Analysis}
We survey ways an adversary can attack our system to learn the private data of parties.
We distinguish between 4 different attacks:
\begin{enumerate}
    \item Cryptographic attacks - attacks against the cryptographic primitives used by the system.
    \item Privacy attacks - black/white-box attacks against the ML models.
    \item Protocol level attacks - attacks against the protocol itself assuming that the implementation has no flaws.
    \item Attacks against the implementation - for example side-channel attacks.
\end{enumerate} 


\subsection{Cryptographic Attacks}
By cryptographic attacks, we refer to adversaries that attempt to attack the cryptographic primitives used by our system. Specifically, we refer to HE and more specifically to CKKS. Other cryptographic primitives are involved only during the secure communication protocol (e.g., TLS 1.3) which we refer to in the following sections. When dealing with cryptographic primitives instead of specifying and evaluating a specific attack we describe a property that basically states what a probable polynomial time (PPT) adversary can expect to achieve no matter how it facilitates the attack.

\begin{itemize}
    \item \textbf{CKKS is semantic security and IND-CPA.} For a given security parameter, every PPT adversary $\mathcal{A}$ who has access to an encryption and evaluation oracles (who can use the public and evaluation keys, respectively), can generate $n$ messages $m_1, \ldots, m_n$ and their encryptions $Enc(m_1), \ldots, Enc(m_n)$, respectively. However, given encryption $Enc(m_0)$ of an additional message $m_0$ unknown to $\mathcal{A}$, it cannot guess $m_0$ with a probability that is non-negligible in the security parameter. 
    
    \textbf{Attacker possible roles:} In our case, $\mathcal{A}$ can be the banks, the aggregator, or every external party who see the ciphertexts or somehow get access to the public/evaluation keys.
    
    \textbf{Extra info} We use the HEAAN CKKS implementation configured with security parameter $\lambda=128$ and we assume that it fulfills the above property.

    \item \textbf{Circuit Privacy.} An HE is considered circuit private if for every PPT adversary $\mathcal{A}$ who holds the HE keys (secret key, public key, and evaluation keys), given a ciphertext $Enc{m} = C(inputs)$ which is the output of a secret circuit, $C$, computed under FHE, $\mathcal{A}$ on secret $inputs$ cannot learn anything about $C$ nor its inputs. 
    Specifically, FHE schemes such as BGV and CKKS are not circuit private. In fact, some works show that the noise encoded in a ciphertext does leak info on the circuit or its inputs. 
    
    \textbf{Attacker possible roles:} In our case, SWIFT holds the secret keys and thus only SWIFT can decrypt ciphertexts and maintain an offline attack to extract the banks data. 
    
    \textbf{Possible mitigation 1:} Ducas and Damien showed a process called {\it sanitization} that randomizes the noise in a ciphertext. After sanitization, no information on $C$ leaks from $Enc(m)$ with overwhelming probability. However, the sanitization process is considered a costly operation, sometimes even unpractical, which our solution avoids. 
    
    \textbf{Possible mitigation 2:} When the message $m$ has some predefined format e.g., integers in the range 1-100. It is possible to modify the decryption to include a round operation before revealing the message to the user \cite{player}. To enable this option, the decryption (+rounding) should be an atomic operation e.g., by running in HW or by executing inside a TEE such as SGX, which is forbidden in the PETs competition. Moreover, the banks need to trust SWIFT and that they indeed perform the decryption only as an atomic operation that they cannot use the secret key to decrypt the data using other computing devices.
    
    \textbf{Remark:} while some works show that it is feasible to extract data from decryption of ciphertexts, we are unaware of any robust attack that can do so for complex circuits.
    
    In the case of circuit privacy, we distinguish between three types of attacks. 
    
    \begin{itemize}
        \item \textbf{Extracting the $inputs$.} An adversary uses the noise in the decrypted plaintexts to extract the $inputs$. For example, when the evaluated circuit $C$ is a NN and the inputs are the model weights. In our case, the circuit is the tree evaluation (training/inference) and the $inputs$ are the flags. As SWIFT already hold this information, we claim that no attack can be maintained for this scenario.
        
        \item \textbf{Extracting $C$.} An adversary uses the noise in the decrypted plaintexts to extract the circuit $C$. In our case, $C$ is the tree evaluation (training/inference). However, $C$ also includes the hash preparation process, which may be different for different banks due to the different number of accounts each one holds or the number of account with a specific value for some flag. 
        
        \textbf{Possible mitigation:} The banks can either agree on a fixed set of computation for all banks, which may artificially limit the number of accounts or includes more than needed computation. Alternatively, we can assume that extracting this information from just the error is hard.
    
        \item \textbf{Error from approximations.} In addition to the encryption noise, some data leaks from the message $m$ itself because we are using polynomial approximations. For example suppose the last step of $C$ is $m := Sign(x)$, where $Sign(x) = 1$ if $x>0$ and $-1$ if $x<0$, then we implement $Sign$ using a polynomial approximation where $m = Sign(x) \in [-1, 1]$ and depends on $x$. This attack can be addressed by either improving the polynomial approximations we use, which may increase the latency, or by adding random noise that is significantly bigger than the error of the approximation, but may hard the results. 
    \end{itemize}
    
    \item \textbf{IND-CPA$^{+}$.} Li and Micciancio showed an attack on IND-CPA CKKS that an adversary who holds an encryption of a message $m$ - $Enc(m)$ and its decryption may be able to extract the secret key. 
    
    \textbf{Attacker possible roles:} The banks, the aggregator, and other third parties, who can collect both ciphertexts and their decryption.
    
    \textbf{Possible mitigation 1:} Many cryptographic libraries already include some mitigation in the form of injecting noise before performing the decryption. Our implementation is based on the HEAAN library and inherits its mitigation if available.
    
    \textbf{Possible mitigation 2:} SWIFT who is the secret key owner should ensure that no decrypted message reaches the hand of the parties above, as they may hold the associated ciphertext. While our code ensures that this is the case, we see the need to re-emphasize it here.
    
    \textbf{Possible mitigation 3:} If SWIFT does not trust the underlying library it can execute a round operation after decryption, which also mitigates the above issue.
    
    \item \textbf{Key management.} We assume that all the keys that are involved in the protocol are stored securely in some Key Management Device (KMS). Currently, our implementation is a stand-alone implementation and thus does not include a KMS. However, we emphasize that special care is needed when handling cryptographic keys.
\end{itemize}


\subsection{Privacy Attacks}
Privacy attacks include two main categories black-box and white-box attacks. The first assumes that an adversary $\mathcal{A}$ gets a black box that implements an ML model, it is able to feed it with a polynomial number of inputs and collect the outputs. Based on the input-output pairs it can learn some private information. A white-box attacker also gets access to some intermediate computation values of the model. Due to the use of CKKS we assume that only black-box attacks are feasible.

\textbf{SWIFT as the attacker:} SWIFT is the main actor who can facilitate privacy attacks, where its goal is to learn the banks' secret data. Note that by SWIFT, we do not only refer to SWIFT acting as a bad actor, which we would like to believe is not the case. Instead, we assume that SWIFT is tricked to maintain the attack under a third-party attacker. 

\textbf{Banks as the attacker:} It is tempting to assume that the banks cannot facilitate privacy attacks as they can only see encrypted data, i.e., they do not get to see the output of the model. However, in a real-life scenario, every SWIFT transaction is triggered by a bank that asks SWIFT to perform this transaction. Thus, a bank can "send inputs" in an attempt to trigger SWIFT to run a model inference operation that eventually will get back to him. This attack is quite hard to do because there is a lot of obfuscating noise - many transactions happen at SWIFT at the same time and it is hard to isolate the input-output pairs.

\textbf{Mitigation} The common mitigation for the below attacks is to use DP.

Some possible attacks are:

\begin{itemize}
    \item \textbf{membership inference attacks}, where $\mathcal{A}$ tries to learn whether a member $x$ was part of the training data. Specifically, whether a specific person is a bank client or whether a transaction happened between different banks
    
    \item \textbf{property extraction attacks.} In this attack, SWIFT may attempt to learn a generic property on the training data of some banks, e.g., whether it has more man clients than women clients.
    
    \item \textbf{model extraction attacks.} While SWIFT knows the model it is unknown to the banks. It may be the case that the banks attempt to extract the model and by that learn what transactions are considered a fraud so that they can cheat SWIFT.
\end{itemize}

\subsection{Protocol level attacks }

Our security proof of the protocol discusses the capabilities of potential adversaries. Specifically, protocol-level attacks take advantage of weaknesses in the protocol to learn non-trivial knowledge.

\begin{itemize}
    \item \textbf{Man-in-the-middle attacks.} In MITM attacks an adversary gets access to the communication between 2 parties in a way that he can replace one message with another. For example, a MITM adversary can replace the messages SWIFT sends the bank or the reply the banks send SWIFT. To protect against MITM attacks always use secure communication between all entities e.g., TLS 1.3. We also assume that there is an agreed certificate authority between the parties for authenticating each other. Our implementation is based on Flower and assumes that it provides secure communication. 
    
    \item \textbf{Malicious adversaries}. Our system assumes the parties are honest-but-curious which means they follow the protocol. Adversaries that deviate from the protocol may influence the output of the protocol or even learn non-trivial information on the private input of the other parties. 
    
    \textbf{Possible mitigation.} To deal with malicious parties zero-knowledge proofs can be embedded in the protocol to prove that at each step the party followed the protocol.
    
    \item \textbf{Malicious input}. To learn something on a specific account $a$, SWIFT might fabricate input involving $a$. This does not fall under the category of a malicious adversary because after fabricating the input SWIFT follows the protocol. 

    \textbf{Possible mitigation.} To address this type of attacks the other parties may ask for a zero-knowledge proof that checks the input is distributed like a real input.
    
    \item Knowing the potential leaves reached by SWIFT.
    
    \item Knowing how many leaves were reached by SWIFT.
\end{itemize}

\subsection{Attacks against the implementation}

This section assumes that the protocol leakage is well defined, e.g., the number of transaction or the number of banks. However, when the protocol was implemented it mistakenly included additional (side-channel) leakage that can be collected by an attacker. 

\begin{itemize}
    \item \textbf{Physical side-channel attacks.} - Because the parties are SWIFT and Banks, we assume that the implementation runs on a computing device in a secure location without physical access to it. Thus, attacks such as power attacks, electromagnetic attacks, acoustic attacks, fault attacks, etc., are outside the scope of our implementation. We also assume that the power measurements cannot be reported by the underlying system (OS, VM) and collected by a remote external attacker. If this is not the case, the implementation must be modified and vetted against these types of attacks.
    
    \item \textbf{Timing attacks on banks: number of accounts.} The number of accounts each bank has is considered a secret. During both the training and the inference time. In addition, the number of accounts that has a specific flag set is also considered a secret. During the pre-processing phase, the protocol asks every bank to compare (hash) all of its accounts, because the number of accounts is different the pre-processing time differs between banks. This can leak the secret account number. 
    
    \textbf{Attacker possible roles} SWIFT, aggregator, third-party entities.

    \textbf{Mitigation} The total execution time depends on the computing equipment every bank has. Thus, we can limit all banks to performing the pre-processing phase in X units of time. Banks that have a low number of accounts and finish the execution after Y units of time can wait for X-Y units of time before returning an answer. Banks that have a large number of accounts should use more computing equipment to meet the X deadline. To meet the 9 hours bar, our implementation does not assume a fixed preprocessing time.
    
    \item \textbf{Timing attacks on SWIFT: number of transactions.} The banks may attempt to infer the number of transactions SWIFT processes every unit of time. This may help them to get better rates with SWIFT. 
    
    \textbf{Attacker possible roles} banks.
    
    \textbf{Mitigation} SWIFT should use the model at frequent times or according to some well, possibly public, known policy. To meet the 9 hours bar, our implementation does not take this info into account.
    
    \item \textbf{}

\end{itemize}



==> generalizing-the-solution.tex <==
\section{Generalizing the Solution}
\label{sec:generalize}

We outline next how to generalize our system to have better prediction accuracy by including additional models such as {\bf logistic regression}.

\vspace{6pt}
\noindent\textbf{Preliminary data alignment and replication step:}
We first generate a unified database including all of SWIFT transactions with details collected from relevant banks. Here, a single account may be {\bf replicated} multiple times if it appears in several transactions. Moreover, in some transactions, it may be the originator and in other transactions, it may be the beneficiary. In addition, accounts that do not participate in transactions will not appear in the database at all.
For privacy reasons, this table is generated using MPC tools including FHE and secret-sharing. The output is also secret-shared and thus no coalition of $k$ parties may read the content of the table, where $k>1$ is a parameter of the protocol. To keep this step efficient with respect to CPU and network we use FHE and secret-sharing, taking the best of each tool.

\vspace{6pt}
\noindent\textbf{Training Over Aligned Data:}
Once we have an aligned and unified dataset we can access it to train various models.
% We now describe a general recipe for {\bf accessing and computing} a function on data from the unified dataset. This recipe is then used to train models.
Accessing is done collaboratively by at least $k$ parties in this manner: 1) a designated party $\mathcal{P}$ is chosen (the designated party may change during the protocol to share the load); 2) At least one of the $k$ parties holding a share encrypts its share and all $k$ parties send their shares to $\mathcal{P}$; 3) $\mathcal{P}$ adds the shares (at least one of whom is encrypted) to get the encrypted value; 4) $\mathcal{P}$ performs the computation over FHE; 5) $\mathcal{P}$ engages with $k$ more parties to create unencrypted random shares of the output.

==> record-alignment-replication.tex <==
\section{Record Alignment and Replication}
\label{sec:recordalginment}



In this section we discuss how Swift and a collection of banks can align their data as a preliminary step before training.
In the beginning of this step Swift has a database of transactions represented as a matrix where each row is a transaction and each column is a transaction feature. In addition, each back has a database of accounts where each row is an account and each column is an account feature.
We think of a database as a matrix $D\in\RR^{r\times c}$ with $r$ rows and $c$ columns. We denote by $D[i,j]$ the $j$th column in the $i$th row. We denote by $D[i]$ the vector in the $i$th row and by $D[*,j]$ the vector in the $j$th column.

We assume there are at most $T$ transactions in Swift's database and that $T$ is known to all banks. We also assume there are at most $A$ accounts in a bank's database and that $A$ is known to Swift and to all banks.

In addition, we assume the parties share an FHE encryption scheme $\E = (\Gen, \Enc, \Dec, \Add, \Mul)$, where each party can generate its own key pair $(sk, pk)$. We denote by Swift key pair by $(sk_s, pk_s)$ and the bank's key pair by $(sk_b, pk_b)$. We denote by $\en{m}_b$ the encryption of a message $m$ with the public key of bank $b$ (different pair for each bank). A message encrypted with Swift's public key is denoted by $\en{m}$. When secret sharing a message $m \in G$, where $G$ is some finite group, we denote the two shares by $\sharea{m}$ and $\shareb{m}$, such that $\sharea{m} + \shareb{m} = m$. In what follows $\sharea{m}$ and $\shareb{m}$ are chosen to be statistically indistinguishable from random (over the group $G$).

{\bf Swift's input}
is a database $\Tdb$ of $T$ transactions (padded with zeroes if needed). Amongst others each transaction $\Tdb[i]$ includes special fields: $\Tdb[*,\swiftsrc]$ the source of the transaction (source bank and originator) and $\Tdb[*,\swiftdst]$ the destination of the transaction (destination bank and beneficiary). 

{\bf Bank $b$'s input}
is a database $\Adb{b}$ of $A$ accounts (padded with zeroes if needed). Amongst others each account include a special field: $\Adb{b}[*,\bankid]$ a unique id of the account (bank id and internal account id).

For the same account, the special fields:
$$(i)\bankid, (ii)\swiftsrc \text {and }(iii)\swiftdst$$
are identical throughout all the databases.



{\bf The output} of the following protocol is a matrix $\Ddb$, where each row corresponds to a transaction. A sub-matrix of $\Ddb$ (some columns) corresponds to the source of transactions and we mark it as $\Dsrc$; another sub-matrix (some columns) corresponds to destination of transactions and we mark it as $\Ddst$ the remaining sub-matrix corresponds to transaction details that are not related to an account, we denote it as $\Dswift$. The matrix $\Ddb$ holds all the transactions. We note that accounts can participate in multiple transactions as originators or beneficiaries. In these cases the account details appears multiple times in $\Ddb$.

{\bf Privacy} is maintained by the protocol by using FHE and secret sharing. The elements of output $\Ddb$ are secret-shared by the parties. That is, each party holds a matrix whose dimensions are identical to $\Ddb$ and is indistinguishable from random, but the sum of all matrices held by the parties is $\Ddb$.

We now describe Protocol~\ref{prot:align}. This protocol is engaged by Swift and a single bank $b$ to generate a subset of $\Ddb$, more specifically the protocol generates subsets of $\Dswift$ and $\Dsrc$ that correspond to transactions originated from $b$.

{\bf Extending to compute the full $\Dswift$ and $\Dsrc$.} As mentioned, Protocol~\ref{prot:align} is engaged by Swift and a single bank $b$ to generate subsets of $\Dswift$ and $\Dsrc$ (denote them as $\Dswift_b$ and $\Dsrc_b$). As constructed by Protocol~\ref{prot:align}, rows of $\Dswift_b$ and $\Dsrc_b$ that do not correspond to transactions originating at bank $b$ are zero. We therefore have the identity $$\Dswift = \sum_b \Dswift_b\text{, and } \Dsrc = \sum_b \Dsrc_b.$$
Therefore, to compute the full matrices $\Dswift$ and $\Dsrc$, Swift needs to add all the shares of $\Dswift_b$ and $\Dsrc_b$ it got into a single share of
$\Dswift$ and $\Dsrc$.


{\bf Extending to compute $\Ddst$.} We note that $\Dsrc$ and $\Ddst$ are symmetrical and it is easy to change Protocol~\ref{prot:align} to compute $\Ddst$ and secret-share it. It is imperative to note that the order in which the transactions appear in $\Ddst$ and $\Dsrc$ is the same. This can be seen in the protocol below since the order is determined by the order in which transactions appear in the hash $H$.

{\bf Reducing number of shares.} After engaging with all banks $\Ddb$ is secret-shared by all banks. Looking forward at the training process we want to keep the communication complexity small and therefore want to reduce the number of parties that hold shares. This can be easily done by aggregating the shares at one designated bank. Since even all the banks together are still missing the share held by Swift, even their aggregated shares is indistinguishable from random. To reduce the load of the designated bank, we can chose a different designated bank for different rows of $\Ddb$.


\begin{algorithm}
\caption{Setup and align}
\label{prot:align}
{\begin{tabbing}
\textbf{Common Parameters:} $T,A\in \NN$, 
$\E = (\Gen, \Enc, \Dec, \Add, \Mul)$ as mentioned in Section~\ref{sec:aligning}\\
\textbf{Parties:} Swift, bank $b$.\\
\textbf{Inputs:} Swift's input: database $\Tdb$. Bank $b$'s input: A database $\Adb{b}$.\\

\textbf{Output:} Swift: $\sharea{\Dsrc_b}$, 
bank $b$: $\shareb{\Dsrc_b}$.\\
\end{tabbing}}

\vspace{-2em}

{\bf Swift performs:}\\
    \quad Insert the ids in $\Tdb[*,\swiftdst]$ and $\Tdb[*,\swiftsrc]$ into a Cuckoo hash $H$ of size $h$ that can accommodate $2T$ entries (as a rule of a thumb $h=4T$). We write the account numbers in the entries of $H$ encoded in binary (each bit encoded in a different ciphertext).
    \quad $\en{H} \assign \Enc(H)$\\
    \quad Send $\en{H}$ to $b$.\\
    \quad Compute a binary matrix $M_S$ such that, $H\cdot M_S = (a_1, \ldots, a_T)$, where $(a_1, \ldots, a_T)$ are the vector of originator account numbers (of all banks) of the transaction (possibly with repetition).\\
    \quad Send $\shareb{M_S} \assign M_S - \sharea{M_S}$ to $b$, where $\sharea{M_S}$ a random $\hashsize\times T$ matrix.\\

{\bf Bank $b$ performs:}\\
    \quad Zeroize a vector $\chi_b \assign 0^\hashsize$ and a matrices $M_b,I_b \assign 0^{\hashsize \times \hashsize}$\\
    \quad \For {$i \in \Adb{b}[i,\bankid]$} {
        \quad \For {hash function $h$} {
            \quad Set $\chi_b[h(i)] \assign \chi_b[h(i)] + \compare{i}{H[h(i)]}$\\
            \quad Set $M_b[i, h(i)] \assign M_b[i, h(i)] + \compare{i}{H[h(i)]}$\\
            \quad Set $I_b[h(i), h(i)] \assign I_b[h(i), h(i)] + \compare{i}{H[h(i)]}$\\
        }
    }
    % \tcc{At this point $\Adb{b} \cdot M_b = H\cdot I_b$}
    \quad $\shareb{I_b} \assign I_b - \sharea{I_b}$, where $\sharea{I_b}$ is a random diagonal matrix.\\
    \quad Send $\en{\sharea{I_b}}_b \assign \Enc(\sharea{I_b})$ to Swift\\
    
{\bf Swift performs:}\\
    \quad $\sharea{\Dsrc_b} \assign \sum_b H \cdot \sharea{I_b} \cdot M_S$\\
    \quad $\en{t}_b \assign H \cdot \en{I_b}_b \cdot \sharea{M_S} + R_b$, where $R_b$ is a random matrix.\\
    \quad Send $\sharea{\Dsrc_b} \assign \sharea{\Dsrc} - R_b$ to bank $b$\\

{\bf Bank $b$ performs:}\\
    \quad $\en{\shareb{\Dsrc_b} + r_b} \assign \Dec(\en{t}_b) + \en{H} \cdot \shareb{I_b} \cdot \shareb{M_S} + r_b$, where $r_b$ is a random matrix.\\
    \quad Send $\en{\shareb{\Dsrc_b} + r_b}$ to Swift\\

{\bf Swift performs:}\\
    \quad Send $(\shareb{\Dsrc_b} + r_b) \assign \Dec(\en{\shareb{\Dsrc} + r_b})$ to bank $b$\\

{\bf Bank $b$ performs:}\\
    \quad $\shareb{\Dsrc_b} \assign (\shareb{\Dsrc} + r_b) - r_b$\\

\end{algorithm}



